A first unbiased global NLO determination of parton distributions and their uncertainties

We present a determination of the parton distributions of the nucleon from a global set of hard scattering data using the NNPDF methodology: NNPDF2.0. Experimental data include deep-inelastic scattering with the combined HERA-I dataset, fixed target Drell-Yan production, collider weak boson production and inclusive jet production. Next-to-leading order QCD is used throughout without resorting to K-factors. We present and utilize an improved fast algorithm for the solution of evolution equations and the computation of general hadronic processes. We introduce improved techniques for the training of the neural networks which are used as parton parametrization, and we use a novel approach for the proper treatment of normalization uncertainties. We assess quantitatively the impact of individual datasets on PDFs. We find very good consistency of all datasets with each other and with NLO QCD, with no evidence of tension between datasets. Some PDF combinations relevant for LHC observables turn out to be determined rather more accurately than in any other parton fit.

==> chi2.tex <==

\begin{table}
\begin{center}
\footnotesize
\begin{tabular}{|c|c|}
\hline 
Experiment  &  $\chi^{2}_{\tot}$ \\
\hline 
\hline
Total           & 1.21 \\
\hline
\hline
NMC-pd          &   0.99\\
\hline
NMC             &   1.69\\
\hline
SLAC            &   1.34 \\
\hline
BCDMS           &   1.27 \\
\hline
HERAI        &   1.14 \\
\hline
CHORUS          &   1.18\\
\hline
FLH108          &   1.49 \\
\hline
NTVDMN          &   0.67 \\
\hline
ZEUS-H2         &   1.51 \\
\hline
DYE605          &   0.88 \\
\hline
DYE866          &   1.28 \\
\hline
CDFWASY         &   1.85 \\
\hline
CDFZRAP         &   2.02 \\
\hline
D0ZRAP          &   0.57 \\
\hline
CDFR2KT         &   0.80 \\
\hline
D0R2CON         &   0.93 \\
\hline
\end{tabular}
\end{center}
\caption{\small The values of the $\chi^2$ for all the experiments
included in the NNPDF2.0 analysis for $N_{\rm rep}=1000$. \label{tab:chi2}}
\end{table}


==> stabtab-20-12.tex <==
\tiny
\begin{tabular}{|c|c|}
\hline
\multicolumn{2}{|c|}{NNPDF2.0 vs. NNPDF1.2} \\
\hline
\hline 
$\Sigma(x,Q_0^2)$ & $5~10^{-4} \le x \le 0.5$   \\
\hline
$\la d[q]\ra$  &  3.0 \\
$\la d[\sigma]\ra$  & 1.7  \\
\hline 
\hline 
$g(x,Q_0^2)$ & $5~10^{-4} \le x \le 0.5$   \\
\hline
$\la d[q]\ra$  &  4.2 \\
$\la d[\sigma]\ra$  & 2.4  \\
\hline 
\hline 
$T_3(x,Q_0^2)$ & $0.03 \le x \le 0.75$   \\
\hline
$\la d[q]\ra$  &  5.4  \\
$\la d[\sigma]\ra$  & 4.1  \\
\hline 
\hline 
$V(x,Q_0^2)$ & $0.01 \le x \le 0.5$    \\
\hline
$\la d[q]\ra$  &  3.1  \\
$\la d[\sigma]\ra$  & 4.1   \\
\hline 
\hline 
$\Delta_S(x,Q_0^2)$ & $0.03 \le x \le 0.5$  
  \\
\hline
$\la d[q]\ra$  & 8.4 \\
$\la d[\sigma]\ra$  &  4.3    \\
\hline 
\hline 
$s^+(x,Q_0^2)$ &  $5~10^{-4} \le x \le 0.1$ \\
\hline
$\la d[q]\ra$  & 1.0  \\
$\la d[\sigma]\ra$  & 1.7    \\
\hline 
\hline 
$s^-(x,Q_0^2)$ & $0.1 \le x \le 0.6$  
 \\
\hline
$\la d[q]\ra$  &  1.9 \\
$\la d[\sigma]\ra$  & 4.1    \\
\hline 
\end{tabular}



==> stabtab-20-dis-jet.tex <==
% --------------------------------------------------------------
\tiny
\begin{tabular}{|c|c|}
\hline
\multicolumn{2}{|c|}{2.0-DIS vs. 2.0-DIS+JET} \\
\hline
\hline 
$\Sigma(x,Q_0^2)$ & $5~10^{-4} \le x \le 0.5$   \\
\hline
$\la d[q]\ra$  & 1.1  \\
$\la d[\sigma]\ra$  & 0.9  \\
\hline 
\hline 
$g(x,Q_0^2)$ & $5~10^{-4} \le x \le 0.5$   \\
\hline
$\la d[q]\ra$  &  2.1 \\
$\la d[\sigma]\ra$  & 1.4  \\
\hline 
\hline 
$T_3(x,Q_0^2)$ & $0.03 \le x \le 0.75$   \\
\hline
$\la d[q]\ra$  & 1.3   \\
$\la d[\sigma]\ra$  & 0.9   \\
\hline 
\hline 
$V(x,Q_0^2)$ & $0.01 \le x \le 0.5$    \\
\hline
$\la d[q]\ra$  &  1.1  \\
$\la d[\sigma]\ra$  & 1.0    \\
\hline 
\hline 
$\Delta_S(x,Q_0^2)$ & $0.03 \le x \le 0.5$  
  \\
\hline
$\la d[q]\ra$  &   1.1 \\
$\la d[\sigma]\ra$  &  1.5     \\
\hline 
\hline 
$s^+(x,Q_0^2)$ &  $5~10^{-4} \le x \le 0.1$ \\
\hline
$\la d[q]\ra$  & 1.4  \\
$\la d[\sigma]\ra$  & 0.9     \\
\hline 
\hline 
$s^-(x,Q_0^2)$ & $0.1 \le x \le 0.6$  
 \\
\hline
$\la d[q]\ra$  & 1.7   \\
$\la d[\sigma]\ra$  & 0.9   \\
\hline 
\end{tabular}
% -----------------------------------------



==> stabtab-20-dis.tex <==
\tiny
\begin{tabular}{|c|c|}
\hline
\multicolumn{2}{|c|}{2.0-DIS vs. 2.0-DIS-HERAold} \\
\hline
\hline 
$\Sigma(x,Q_0^2)$ & $5~10^{-4} \le x \le 0.5$   \\
\hline
$\la d[q]\ra$  & 1.1  \\
$\la d[\sigma]\ra$  & 1.0  \\
\hline 
\hline 
$g(x,Q_0^2)$ & $5~10^{-4} \le x \le 0.5$   \\
\hline
$\la d[q]\ra$  & 2.2  \\
$\la d[\sigma]\ra$  & 1.2  \\
\hline 
\hline 
$T_3(x,Q_0^2)$ & $0.03 \le x \le 0.75$   \\
\hline
$\la d[q]\ra$  &  1.4  \\
$\la d[\sigma]\ra$  & 0.9  \\
\hline 
\hline 
$V(x,Q_0^2)$ & $0.01 \le x \le 0.5$    \\
\hline
$\la d[q]\ra$  &  1.0  \\
$\la d[\sigma]\ra$  & 1.0    \\
\hline 
\hline 
$\Delta_S(x,Q_0^2)$ & $0.03 \le x \le 0.5$  
  \\
\hline
$\la d[q]\ra$  &   2.1\\
$\la d[\sigma]\ra$  & 2.2     \\
\hline 
\hline 
$s^+(x,Q_0^2)$ &  $5~10^{-4} \le x \le 0.1$ \\
\hline
$\la d[q]\ra$  &  1.4 \\
$\la d[\sigma]\ra$  & 1.0     \\
\hline 
\hline 
$s^-(x,Q_0^2)$ & $0.1 \le x \le 0.6$  
 \\
\hline
$\la d[q]\ra$  &  0.8  \\
$\la d[\sigma]\ra$  & 0.8   \\
\hline 
\end{tabular}



==> stabtab-20-heraold.tex <==
\tiny
\begin{tabular}{|c|c|}
\hline
\multicolumn{2}{|c|}{2.0 vs. 2.0-HERAold} \\
\hline
\hline 
$\Sigma(x,Q_0^2)$ & $5~10^{-4} \le x \le 0.5$   \\
\hline
$\la d[q]\ra$  &  1.5 \\
$\la d[\sigma]\ra$  & 1.2   \\
\hline 
\hline 
$g(x,Q_0^2)$ & $5~10^{-4} \le x \le 0.5$   \\
\hline
$\la d[q]\ra$  & 2.7  \\
$\la d[\sigma]\ra$  & 1.0   \\
\hline 
\hline 
$T_3(x,Q_0^2)$ & $0.03 \le x \le 0.75$   \\
\hline
$\la d[q]\ra$  & 1.0   \\
$\la d[\sigma]\ra$  & 1.1  \\
\hline 
\hline 
$V(x,Q_0^2)$ & $0.01 \le x \le 0.5$    \\
\hline
$\la d[q]\ra$  & 1.3   \\
$\la d[\sigma]\ra$  & 1.0    \\
\hline 
\hline 
$\Delta_S(x,Q_0^2)$ & $0.03 \le x \le 0.5$  
  \\
\hline
$\la d[q]\ra$  &  0.9 \\
$\la d[\sigma]\ra$  & 1.1     \\
\hline 
\hline 
$s^+(x,Q_0^2)$ &  $5~10^{-4} \le x \le 0.1$ \\
\hline
$\la d[q]\ra$  &  1.3 \\
$\la d[\sigma]\ra$  &  1.3     \\
\hline 
\hline 
$s^-(x,Q_0^2)$ & $0.1 \le x \le 0.6$  
 \\
\hline
$\la d[q]\ra$  &   0.9 \\
$\la d[\sigma]\ra$  & 0.9  \\
\hline 
\end{tabular}



==> stabtab-20-ref-dis-jet.tex <==
\tiny
\begin{tabular}{|c|c|}
\hline
\multicolumn{2}{|c|}{2.0 vs. 2.0-DIS+JET} \\
\hline
\hline 
$\Sigma(x,Q_0^2)$ & $5~10^{-4} \le x \le 0.5$   \\
\hline
$\la d[q]\ra$  & 1.5 \\
$\la d[\sigma]\ra$  & 1.0  \\
\hline 
\hline 
$g(x,Q_0^2)$ & $5~10^{-4} \le x \le 0.5$   \\
\hline
$\la d[q]\ra$  & 1.7 \\
$\la d[\sigma]\ra$  & 1.0  \\
\hline 
\hline 
$T_3(x,Q_0^2)$ & $0.03 \le x \le 0.75$   \\
\hline
$\la d[q]\ra$  &  6.5  \\
$\la d[\sigma]\ra$  & 1.6   \\
\hline 
\hline 
$V(x,Q_0^2)$ & $0.01 \le x \le 0.5$    \\
\hline
$\la d[q]\ra$  &  5.6  \\
$\la d[\sigma]\ra$  & 2.6     \\
\hline 
\hline 
$\Delta_S(x,Q_0^2)$ & $0.03 \le x \le 0.5$  
  \\
\hline
$\la d[q]\ra$  &  4.3 \\
$\la d[\sigma]\ra$  & 4.8      \\
\hline 
\hline 
$s^+(x,Q_0^2)$ &  $5~10^{-4} \le x \le 0.1$ \\
\hline
$\la d[q]\ra$  &  1.2 \\
$\la d[\sigma]\ra$  &  1.0     \\
\hline 
\hline 
$s^-(x,Q_0^2)$ & $0.1 \le x \le 0.6$  
 \\
\hline
$\la d[q]\ra$  & 5.0   \\
$\la d[\sigma]\ra$  & 3.5    \\
\hline 
\end{tabular}


